Bayesian Meta-Learning for Few-Shot Policy Adaptation Across Robotic Platforms

Reinforcement learning methods can achieve significant performance but require a large amount of training data collected on the same robotic platform. A policy trained with expensive data is rendered useless after making even a minor change to the robot hardware. In this paper, we address the challenging problem of adapting a policy, trained to perform a task, to a novel robotic hardware platform given only few demonstrations of robot motion trajectories on the target robot. We formulate it as a few-shot meta-learning problem where the goal is to find a meta-model that captures the common structure shared across different robotic platforms such that data-efficient adaptation can be performed. We achieve such adaptation by introducing a learning framework consisting of a probabilistic gradient-based meta-learning algorithm that models the uncertainty arising from the few-shot setting with a low-dimensional latent variable. We experimentally evaluate our framework on a simulated reaching and a real-robot picking task using 400 simulated robots generated by varying the physical parameters of an existing set of robotic platforms. Our results show that the proposed method can successfully adapt a trained policy to different robotic platforms with novel physical parameters and the superiority of our meta-learning algorithm compared to state-of-the-art methods for the introduced few-shot policy adaptation problem.

==> tables/scenario1.tex <==
\begin{table*}[t]
    \centering
    \caption{The average, best and standard deviation of the reaching error (in cm) of the adapted policies. The meta-learner is trained and tested on the data generated by the same platform as in scenario (a). \emph{Y} stands for YuMi, \emph{B} for Baxter, \emph{K} for Kinova, and \emph{F} for Franka Emika, while the numbers denote the index of the test robot. 
    %to three novel robots built on the four platforms, \emph{Y} for YuMi, \emph{B} for Baxter, \emph{K} for Kinova, and \emph{F} for Franka Emika. The meta-learner is trained and tested on the data generated by the same platform as described in scenario 1. 
    }
    \begin{tabular}{l l|l|l|l|l|l|l|l|l|l|l|l|l}
    %\hline
         & & \emph{Y1} & \emph{Y2} &\emph{Y3} & \emph{B1} & \emph{B2} & \emph{B3} & \emph{K1} & \emph{K2} & \emph{K3}  & \emph{F1} & \emph{F2} & \emph{F3} \\
        \hline
        \textbf{Ours} & average & \textbf{1.16} & \textbf{1.71} & \textbf{1.08} & \textbf{0.63} & \textbf{0.59} & 1.39 & \textbf{0.38} & \textbf{1.23} & \textbf{1.02} & \textbf{0.64} & \textbf{1.25} & \textbf{0.68} \\
        \cline{2-14}
          & best & 1.06 & \textbf{1.57} & 0.94 & \textbf{0.44} & \textbf{0.51} & 1.36 & 0.28 & \textbf{1.02} & \textbf{0.85} & 0.47 & 1.09 & 0.49 \\
        \cline{2-14}
          & std & 0.08 & 0.15 & 0.07 & 0.08 & 0.04 & 0.02 & 0.10 & 0.15 & 0.08 & 0.06 & 0.08 & 0.10 \\
        \hline        
        \textbf{AVI} & average & 2.55 & 2.58 & 1.66 & 1.99 & 4.11 & 1.74 & 1.14 & 3.19 & 3.64 & 1.39 & 2.06 & 1.46 \\
        \cline{2-14}
          & best & 1.15 & 1.79 & 0.95 & 0.88 & 1.60 & \textbf{0.50} & \textbf{0.20} & 2.37 & 3.19 & \textbf{0.41} & \textbf{0.73} & \textbf{0.26} \\
        \cline{2-14}
          & std & 1.29 & 0.43 & 0.93 & 0.73 & 1.36 & 0.62 & 0.79 & 0.62 & 0.50 & 0.64 & 0.90 & 1.41 \\
          
        \hline        
        \textbf{VERSA} & average & 1.58 & 3.66 & 1.36 & 1.50 & 2.72 & \textbf{1.22} & 1.36 & 1.58 & 1.85 & 1.32 & 2.06 & 1.54 \\
        \cline{2-14}
          & best & \textbf{0.92} & 2.35 & \textbf{0.93} & 0.59 & 0.86 & 0.77 & 0.51 & 1.20 & 0.97 & 0.89 & 0.75 & 0.53 \\
        \cline{2-14}
          & std & 0.49 & 1.18 & 0.24 & 0.83 & 0.88 & 0.29 & 0.42 & 0.28 & 0.43 & 0.42 & 1.05 & 0.65 \\   
          
        \hline
        \textbf{MAML} &  & 1.88 & 3.05 & 2.13 & 0.55 & 1.09 & 1.63 & 0.50 & 1.16 & 1.24 & 1.52 & 0.81 & 1.19
        %\hline
    \end{tabular}
    \label{tabel:exp:scenario1}
\end{table*}

==> tables/scenario2.tex <==
\begin{table*}[t]
    \centering
    \caption{The average, best and standard deviation of the reaching error as in Table \ref{tabel:exp:scenario1}.
    %of the adapted policy to three novel robots built on the four platforms. 
    The meta-learner is trained and tested on the data generated by all four platforms as in scenario (b). }
    \begin{tabular}{l l|l|l|l|l|l|l|l|l|l|l|l|l}
    %\hline
         & & \emph{Y1} & \emph{Y2} &\emph{Y3} & \emph{B1} & \emph{B2} & \emph{B3} & \emph{K1} & \emph{K2} & \emph{K3}  & \emph{F1} & \emph{F2} & \emph{F3} \\
        \hline
        \textbf{Ours} & average & \textbf{1.14} & \textbf{1.44} & \textbf{0.91} & \textbf{0.86} & \textbf{2.48} & 2.57 & \textbf{0.45} & \textbf{0.84} & \textbf{0.94} & 1.92 & \textbf{1.37} & \textbf{1.40} \\
        \cline{2-14}
          & best & 1.00 & \textbf{1.37} & \textbf{0.72} & 0.52 & 0.91 & 1.73 & \textbf{0.36} & 0.76 & 0.88 & 1.21 & 0.76 & 0.97 \\
        \cline{2-14}
          & std & 0.13 & 0.04 & 0.17 & 0.33 & 2.02 & 1.00 & 0.06 & 0.05 & 0.04 & 0.54 & 0.70 & 0.33 \\
        \hline        
        \textbf{AVI} & average & 1.75 & 4.06 & 1.55 & 1.43 & 6.04 & 1.50 & 1.98 & 1.76 & 1.65 & 2.51 & 1.78 & 2.00 \\
        \cline{2-14}
          & best & \textbf{0.82} & 2.77 & 1.33 & 0.49 & 3.99 & \textbf{0.47} & 0.96 & 0.73 & \textbf{0.66} & 0.95 & \textbf{0.60} & 0.69 \\
        \cline{2-14}
          & std & 0.51 & 1.19 & 0.15 & 0.70 & 1.47 & 1.41 & 0.63 & 0.48 & 0.63 & 1.12 & 0.86 & 1.28 \\
          
        \hline        
        \textbf{VERSA} & average & 2.66 & 4.29 & 1.38 & 1.46 & 3.40 & \textbf{1.11} & 1.64 & 1.59 & 2.47 & \textbf{1.51} & 2.16 & 1.48 \\
        \cline{2-14}
          & best & 2.23 & 2.47 & 1.02 & \textbf{0.47} & \textbf{0.53} & 0.55 & 1.05 & \textbf{0.64} & 2.33 & \textbf{0.62} & 0.77 & \textbf{0.53} \\
        \cline{2-14}
          & std & 0.26 & 1.26 & 0.23 & 0.79 & 1.74 & 0.58 & 0.42 & 0.53 & 0.10 & 0.86 & 0.73 & 0.62 \\        
        
        \hline
        \textbf{MAML} &  & 8.76 & 7.35 & 7.61 & 4.99 & 5.74 & 5.58 & 5.89 & 6.19 & 6.05 & 6.28 & 6.17 & 6.35 \\
        %\hline
    \end{tabular}
    \label{tabel:exp:scenario2}
\end{table*}

==> tables/scenario3.tex <==
\begin{table*}[t]
    \centering
    \caption{
    The average, best and standard deviation of the reaching error as in Table \ref{tabel:exp:scenario1}.
    %The average reaching error of the adapted policy to three novel robots built on the four platforms. 
    The meta-learner is trained on the data from all platforms except the one that is used for meta-testing as described in scenario (c).}
    \begin{tabular}{l l|l|l|l|l|l|l|l|l|l|l|l|l}
    %\hline
         & & \emph{Y1} & \emph{Y2} &\emph{Y3} & \emph{B1} & \emph{B2} & \emph{B3} & \emph{K1} & \emph{K2} & \emph{K3}  & \emph{F1} & \emph{F2} & \emph{F3} \\
        \hline
        \textbf{Ours} & average & \textbf{9.63} & \textbf{10.30} & \textbf{9.67} & \textbf{5.91} & \textbf{11.58} & 17.30 & \textbf{22.57} & 26.40 & \textbf{23.59} & 16.53 & 18.07 & 15.24 \\
        \cline{2-14}
          & best & \textbf{9.29} & \textbf{10.20} & \textbf{9.51} & \textbf{3.92} & \textbf{3.73}  & \textbf{8.43}  & \textbf{20.81} & 21.03 & \textbf{17.70} & \textbf{14.02} & \textbf{14.95} & \textbf{13.18} \\
        \cline{2-14}
          & std & 0.39 & 0.09  & 0.37 & 3.00 & 6.20  & 7.33  & 1.98  & 4.66  & 3.01  & 1.06  & 1.03  & 1.14  \\
        \hline        
        \textbf{AVI} & average & 11.44 & 11.12 & 11.13 & 8.13 & 16.64 & 23.59 & 24.95 & \textbf{26.13} & 30.11 & 31.97 & 31.97 & 31.97 \\
        \cline{2-14}
          & best & 10.27 & 10.24 & 10.38 & 7.70 & 13.63 & 12.78 & 20.84 & \textbf{20.75} & 23.29 & 31.97 & 31.97 & 31.97 \\
        \cline{2-14}
          & std & 1.41  & 1.42  & 0.55  & 0.26 & 1.30  & 7.02  & 3.93  & 4.37  & 5.25  & 0.00  & 0.00  & 0.00  \\
          
        \hline        
        \textbf{VERSA} & average & 10.37 & 10.60 & 11.18 & 8.65 & 15.87 & \textbf{14.01} & 25.17 & 32.74 & 29.34 & 31.97 & 31.97 & 31.97  \\
        \cline{2-14}
          & best & 10.17 & 10.24 & 10.34 & 7.80 & 14.64 & 10.63 & 23.78 & 30.65 & 28.46 & 31.97 & 31.97 & 31.97 \\
        \cline{2-14}
          & std & 0.16  & 0.35  & 0.43  & 0.63 & 0.85  & 1.15  & 0.98  & 1.50  & 0.45  & 0.00  & 0.00  & 0.00 \\             
          
        \hline
        \textbf{MAML} &  & 10.86 & 17.42 & 16.20 & 23.41 & 25.85 & 15.51 & 30.79 & 33.65 & 29.17 & \textbf{12.66} & \textbf{12.42} & \textbf{13.26}
        %\hline
        %\hline
    \end{tabular}
    \label{tabel:exp:scenario3}
\end{table*}
